The Mathematical Structure of Integrated Information Theory

Integrated Information Theory is one of the leading models of consciousness. It aims to describe both the quality and quantity of the conscious experience of a physical system, such as the brain, in a particular state. In this contribution, we propound the mathematical structure of the theory, separating the essentials from auxiliary formal tools. We provide a definition of a generalized IIT which has IIT 3.0 of Tononi et. al., as well as the Quantum IIT introduced by Zanardi et. al. as special cases. This provides an axiomatic definition of the theory which may serve as the starting point for future formal investigations and as an introduction suitable for researchers with a formal background.

==> 1_conclusion.tex <==
\section{Conclusion}

We could say something about: (But not sure whether this makes sense.)
- central identity of classical IIT and relation to cause-effect repertoire
- possibility to consider simpler cause-effect repertoires
- point to process theories again and to further examples (quantum / leaking) in other paper
- say something about meaning of the crucial steps (probably rather not)
- Repertoires: In IIT 3.0, this map is defined in terms of dynamical properties of the system.
- q-shape describing the \emph{quality} of the systems experience.		
- List new mathematical problems in our Outlook (existence, non-uniqueness, behaviour over coarse-graining, stability)

Outlook / usefulness of this reconstruction:
- shown: solve math problems
- could include lower bound thing
- control over the behaviour of the theory
- our major hope: guidance in the further development of the theory


For later use:
- Product of proto-spaces = compositional structure of experience (?)
- Proto space first, map is second.
In classical IIT, this is intertwined
